AE-NeRF: Auto-Encoding Neural Radiance Fields for 3D-Aware Object Manipulation

We propose a novel framework for 3D-aware object manipulation, called Auto-Encoding Neural Radiance Fields (AE-NeRF). Our model, which is formulated in an auto-encoder architecture, extracts disentangled 3D attributes such as 3D shape, appearance, and camera pose from an image, and a high-quality image is rendered from the attributes through disentangled generative Neural Radiance Fields (NeRF). To improve the disentanglement ability, we present two losses, global-local attribute consistency loss defined between input and output, and swapped-attribute classification loss. Since training such auto-encoding networks from scratch without ground-truth shape and appearance information is non-trivial, we present a stage-wise training scheme, which dramatically helps to boost the performance. We conduct experiments to demonstrate the effectiveness of the proposed model over the latest methods and provide extensive ablation studies.

==> figures/auto-encoding-chairs.tex <==
\begin{figure*}[!t]
\centering
\begin{tabular}{M{0.06\linewidth} M{0.9\linewidth}}
& 
{\includegraphics[width=0.11\linewidth]{clipnerf/real1.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/real2.png}}\hfill 
{\includegraphics[width=0.11\linewidth]{clipnerf/real3.png}}\hfill 
{\includegraphics[width=0.11\linewidth]{clipnerf/real4.png}}\hfill 
{\includegraphics[width=0.11\linewidth]{clipnerf/real5.png}}\hfill 
{\includegraphics[width=0.11\linewidth]{clipnerf/real6.png}}\hfill 
{\includegraphics[width=0.11\linewidth]{clipnerf/real7.png}}\hfill 
{\includegraphics[width=0.11\linewidth]{clipnerf/real8.png}}\hfill 
\\

\rotatebox{90}{\makecell{Clip \\ NeRF}} &
{\includegraphics[width=0.11\linewidth]{clipnerf/clip1.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/clip2.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/clip3.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/clip4.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/clip5.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/clip6.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/clip7.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf/clip8.png}}\hfill\\

\rotatebox{90}{Ours} &
{\includegraphics[width=0.11\linewidth]{clipnerf_comparison/1_rgb.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf_comparison/2_rgb.png}}\hfill
{\includegraphics[width=0.11\linewidth]{example-image}}\hfill 
{\includegraphics[width=0.11\linewidth]{example-image}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf_comparison/5_rgb.png}}\hfill
{\includegraphics[width=0.11\linewidth]{clipnerf_comparison/6_rgb.png}}\hfill 
{\includegraphics[width=0.11\linewidth]{example-image}}\hfill
{\includegraphics[width=0.11\linewidth]{example-image}}\hfill \\
\end{tabular}

\caption{3D reconstruction comparison with ClipNeRF on CARLA and Photoshapes dataset.}
\label{auto-encoding-chairs}
\end{figure*}


==> figures/extrapolation2.tex <==
\begin{figure*}[!tp]
\begin{minipage}[t][\textheight]{\linewidth}
\centering
\begin{center}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\vspace{2cm}
\begin{tabular}{M{0.10\linewidth} c M{0.64\linewidth} M{0.10\linewidth}}
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{extrapolation/79_153/0_gt.png}\hfill } \\  Image 1 \\ 
\end{tabular}  }
& 
sh. &
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_shape_7.png}} &
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{extrapolation/79_153/1_gt.png}\hfill } \\  Image 2 
\end{tabular}  }
\\ 
& app. & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_app_7.png}} &
\\
& cam. & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_cam_7.png}} &
\\
& all & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/editnerf/edit_all_7.png}} &
\\ [-5pt]
& &\multicolumn{1}{c}{$\xleftarrow{\hspace*{1.05cm}}$ extra. $\xrightarrow{\hspace*{1.05cm}}$ $\xleftarrow{\hspace*{1.05cm}}$ inter. $\xrightarrow{\hspace*{1.05cm}}$ $\xleftarrow{\hspace*{1.05cm}}$ extra. $\xrightarrow{\hspace*{1.05cm}}$ }& \\[10pt] % 이게 그 두 interpolation 구분하는 간격

\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{extrapolation/79_153/0_gt.png}\hfill } \\  Image 1 \\ 
\end{tabular}  }
& 
sh. &
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_7.png}} &
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{extrapolation/79_153/1_gt.png}\hfill } \\  Image 2 
\end{tabular}  }
\\ 
& app. & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_7.png}} &
\\
& cam. & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_7.png}} &
\\
& all & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_7.png}} &
\\ [-5pt]
& &\multicolumn{1}{c}{$\xleftarrow{\hspace*{1.05cm}}$ extra. $\xrightarrow{\hspace*{1.05cm}}$ $\xleftarrow{\hspace*{1.05cm}}$ inter. $\xrightarrow{\hspace*{1.05cm}}$ $\xleftarrow{\hspace*{1.05cm}}$ extra. $\xrightarrow{\hspace*{1.05cm}}$ }& \\


\end{tabular}

\end{center}
\vspace{-5pt}
\caption{\textbf{Comparison of attribute extrapolation between (top) EditNeRF~\cite{liu2021editing} and (bottom) AE-NeRF}. We extrapolate shape, appearance, camera viewpoint attribute between two images. Given two different images, our AE-NeRF smoothly interpolates the generated images within real data distribution as well as disentangles the shape, appearance, and camera poses, while EditNeRF~\cite{liu2021editing} often fails.}
\label{extrapolation example}
\vspace{10pt}
\begin{center}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{M{0.10\linewidth} c M{0.64\linewidth} M{0.10\linewidth}}
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{extrapolation/79_153/0_gt.png}\hfill } \\  Image 1 \\ 
\end{tabular}  }
& 
sh. &
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/shape_7.png}} &
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{extrapolation/79_153/1_gt.png}\hfill } \\  Image 2 
\end{tabular}  }
\\ 
& app. & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/app_7.png}} &
\\
& cam. & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/pose_7.png}} &
\\
& all & 
\centering
{\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_0.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_1.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/0_recon.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_2.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_3.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_4.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_5.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_6.png}
\includegraphics[width=0.1\linewidth]{extrapolation/79_153/all_7.png}} &
\\ [-5pt]
& &\multicolumn{1}{c}{$\xleftarrow{\hspace*{1.05cm}}$ extra. $\xrightarrow{\hspace*{1.05cm}}$ $\xleftarrow{\hspace*{1.05cm}}$ inter. $\xrightarrow{\hspace*{1.05cm}}$ $\xleftarrow{\hspace*{1.05cm}}$ extra. $\xrightarrow{\hspace*{1.05cm}}$ }& \\



\end{tabular}
\end{center}
\vspace{-10pt}
\caption{\textbf{Attribute extrapolation of AE-NeRF.} We extrapolate shape, appearance, camera viewpoint attribute between two images from the Photoshapes dataset.}
\label{extrapolation example}\vspace{-5pt}
\end{minipage}
\end{figure*}
% \end{fullpagefigure*}

==> figures/interpolation2.tex <==
\begin{figure*}[!tp]
\begin{minipage}[t][\textheight]{\linewidth}
\centering
\begin{center}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\vspace{2cm}
\begin{tabular}{M{0.10\linewidth} c M{0.64\linewidth} M{0.10\linewidth}}
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{interpolation/editnerf/0191_gt.png}\hfill } \\  Image 1 \\ 
\end{tabular}  }
& 
sh. &
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/editnerf/0191_rgb.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_shape_7.png}
} &
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{interpolation/editnerf/0205_gt.png}\hfill } \\  Image 2 
\end{tabular}  }
\\ 
& app. & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/editnerf/0191_rgb.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_app_7.png}
} &
\\
& cam. & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/editnerf/0191_rgb.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_cam_7.png}} &
\\
& all & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/editnerf/0191_rgb.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/editnerf/edit_all_7.png}} &
\\ [-5pt]
& & \multicolumn{1}{c}{$\xleftarrow{\hspace*{3.9cm}}$ interpolation ratio $\xrightarrow{\hspace*{3.9cm}}$}& \\
\end{tabular}
\begin{tabular}{M{0.10\linewidth} c M{0.64\linewidth} M{0.10\linewidth}}
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{interpolation/191_205/0_gt.png}\hfill } \\  Image 1 \\ 
\end{tabular}  }
& 
sh. &
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/0_shape.png}} &
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{interpolation/191_205/1_gt.png}\hfill } \\  Image 2 
\end{tabular}  }
\\ 
& app. & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/0_app.png}} &
\\
& cam. & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/0_pose.png}} &
\\
& all & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/1_recon.png}} &
\\ [-5pt]
& & \multicolumn{1}{c}{$\xleftarrow{\hspace*{3.9cm}}$ interpolation ratio $\xrightarrow{\hspace*{3.9cm}}$}&  \\
\vspace{10pt} % 이게 그 두 interpolation 구분하는 간격
\end{tabular}
\vspace{-5pt}
\caption{\textbf{Comparison of attribute interpolation between (top) EditNeRF~\cite{liu2021editing} and (bottom) AE-NeRF}. We interpolate shape, appearance, camera viewpoint attribute between two images. Given two different images, our AE-NeRF smoothly interpolates the generated images within real data distribution as well as disentangles the shape, appearance, and camera poses, while EditNeRF~\cite{liu2021editing} often fails.}
\label{interpolation example}
\vspace{10pt}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{M{0.10\linewidth} c M{0.64\linewidth} M{0.10\linewidth}}
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{interpolation/191_205/0_gt.png}\hfill } \\  Image 1 \\ 
\end{tabular}  }
& 
sh. &
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/shape_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/0_shape.png}} &
\multirow{8}{*}{\begin{tabular}{c} 
{\includegraphics[width=0.8\linewidth]{interpolation/191_205/1_gt.png}\hfill } \\  Image 2 
\end{tabular}  }
\\ 
& app. & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/app_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/0_app.png}} &
\\
& cam. & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/pose_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/0_pose.png}} &
\\
& all & 
\centering
{\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_0.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_1.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_2.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_3.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_4.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_5.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_6.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/all_7.png}
\includegraphics[width=0.1\linewidth]{interpolation/191_205/1_recon.png}} &
\\ [-5pt]
& & \multicolumn{1}{c}{$\xleftarrow{\hspace*{3.9cm}}$ interpolation ratio $\xrightarrow{\hspace*{3.9cm}}$}&  \\
\vspace{10pt} % 이게 그 두 interpolation 구분하는 간격
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{\textbf{Attribute interpolation of AE-NeRF}. We interpolate shape, appearance, camera viewpoint attribute between two images from the Photoshapes dataset.}
\label{interpolation_chairs}\vspace{-5pt}
\end{minipage}
\end{figure*}%\clearpage


==> figures/novel_view_synthesis.tex <==
\begin{figure*}[t!]
  \centering
  \renewcommand{\thesubfigure}{}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/shape_1_src.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/shape_1_tgt.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/shape_1_rst.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/app_1_src.png}} \hfill \hspace{7pt}
    \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/app_1_tgt.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/app_1_rst.png}} \hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/pose_1_src.png}}\hfill \hspace{-2pt}
    \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/pose_1_tgt.png}}\hfill \hspace{7pt}\hfill\\
  %\vspace{-20pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/shape_2_src.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/shape_2_tgt.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/shape_2_rst.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/app_2_src.png}} \hfill \hspace{7pt}
    \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/app_2_tgt.png}}\hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/app_2_rst.png}} \hfill \hspace{-2pt}
  \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/pose_2_src.png}}\hfill \hspace{-2pt}
    \subfigure[]
  {\includegraphics[width=0.1\linewidth]{dataset/pose_2_tgt.png}}\hfill \hspace{7pt}\hfill\\
  \vspace{-20pt}
\caption{\textbf{Qualitative comparison of novel view synthesis on proposed test dataset of CARLA~\cite{dosovitskiy2017carla} benchmark.} Given source images (col. 1 and 5), we compare the results of novel view synthesis by PixelNeRF~\cite{yu2021PixelNeRF} (row 1) which use ground truth camera pose and AE-NeRF (row 2) which utilize the aligned camera pose for the coordinate system of our decoder.}
\label{PixelNeRF_comparison}%\vspace{-10pt}
\end{figure*}

==> figures/optimization.tex <==
% \begin{figure}[t!]
%   \centering
%   \renewcommand{\thesubfigure}{}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/shape_1_src.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/shape_1_tgt.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/shape_1_rst.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/app_1_src.png}} \hfill \hspace{7pt}\hfill\\
%     \vspace{-20pt}
%     \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/app_1_tgt.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/app_1_rst.png}} \hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/pose_1_src.png}}\hfill \hspace{-2pt}
%     \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/pose_1_tgt.png}}\hfill \hspace{7pt}\hfill\\
%   \vspace{-20pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/shape_2_src.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/shape_2_tgt.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/shape_2_rst.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/app_2_src.png}} \hfill \hspace{7pt}\hfill\\
%     \vspace{-20pt}
%     \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/app_2_tgt.png}}\hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/app_2_rst.png}} \hfill \hspace{-2pt}
%   \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/pose_2_src.png}}\hfill \hspace{-2pt}
%     \subfigure[]
%   {\includegraphics[width=0.2\linewidth]{dataset/pose_2_tgt.png}}\hfill \hspace{7pt}\hfill\\
%   \vspace{-20pt}
% \caption{\textbf{Comparison on test time optimization.} We extract the subset of CARLA~\cite{dosovitskiy2017carla} benchmark to measure the test time optimization quality of models. Given images (columns 1 and 5), we show the results: CodeNeRF (columns 2 and 6), EditNeRF (columns 3 and 7) and AE-NeRF (columns 4 and 8) which renders the rays at test time.}
% \label{fig:test time optimization}\vspace{-5pt}
% \end{figure}
